Disentangling Dense Multi-Cable Knots

Disentangling two or more cables requires many steps to remove crossings between and within cables. We formalize the problem of disentangling multiple cables and present an algorithm, Iterative Reduction Of Non-planar Multiple cAble kNots (IRON-MAN), that outputs robot actions to remove crossings from multi-cable knotted structures. We instantiate this algorithm with a learned perception system, inspired by prior work in single-cable untying that given an image input, can disentangle two-cable twists, three-cable braids, and knots of two or three cables, such as overhand, square, carrick bend, sheet bend, crown, and fisherman's knots. IRON-MAN keeps track of task-relevant keypoints corresponding to target cable endpoints and crossings and iteratively disentangles the cables by identifying and undoing crossings that are critical to knot structure. Using a da Vinci surgical robot, we experimentally evaluate the effectiveness of IRON-MAN on untangling multi-cable knots of types that appear in the training data, as well as generalizing to novel classes of multi-cable knots. Results suggest that IRON-MAN is effective in disentangling knots involving up to three cables with 80.5% success and generalizing to knot types that are not present during training, with cables of both distinct or identical colors.

==> 0-macros.tex <==
%\usepackage{amsmath,graphics}
%\usepackage{amssymb} 
%\usepackage{nicefrac, multirow}
%\usepackage{algpseudocode}
%\usepackage[linesnumbered]{algorithm2e}
%\usepackage{tikz}
%\usepackage{bigstrut}
\setlength\bigstrutjot{3pt}
%\usepackage{pgfplots}
% \pgfplotsset{compat=newest}
%\usepackage{subfig}
%\usepackage{textcomp}
%\usepackage{wrapfig}
\usetikzlibrary{backgrounds}
\numberwithin{equation}{section} 
%\newtheorem{thm}{Theorem}[section]  
%\newtheorem{cor}[thm]{Corollary}    % Corollary environment
%\newtheorem{lem}[thm]{Lemma}        % Lemma environment
%\newtheorem{dfn}[thm]{Definition}        % Lemma environment
%\newtheorem{prop}[thm]{Proposition}  % Proposition environment
%\newtheorem{rem}[thm]{Remark}  % Proposition environment
%\newtheorem{con}[thm]{Conjecture}  % Proposition environment
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\ceq}{\ensuremath{\mathrel{\stackrel{\mathrm{def}}{=}}}} 
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\rd}{{\mathrm d}}
\newcommand{\p}{\partial}
\tikzstyle{every node}=[font=\small]
%%\usepackage{filemod}
\newcommand{\includetikz}[2]{%
\tikzsetnextfilename{#2}%
    \filemodCmp{#1#2.tikz}{#1tikz/#2.pdf}%
        {\tikzset{external/remake next}}{}%
    \input{#1#2.tikz}%
}

\captionsetup{font={footnotesize}}

%\usepackage{tabularx}
%\usepackage{pbox}
%\usepackage{ragged2e}
%\usepackage{multirow}
%\usepackage{floatrow}
% Table float box with bottom caption, box width adjusted to content
% \newfloatcommand{capbtabbox}{table}[][\FBwidth]

\newcolumntype{L}[1]{>{\RaggedRight\hspace{0pt}}p{#1}}
\newcolumntype{R}[1]{>{\RaggedLeft\hspace{0pt}}p{#1}}

\DeclareMathOperator{\J}{J} 
\DeclareMathOperator{\clamp}{clamp} 
\DeclareMathOperator{\interior}{int} 
\DeclareMathOperator{\D}{D} 
\DeclareMathOperator{\Div}{div} 
\DeclareMathOperator{\Sgn}{Sgn} 
\DeclareMathOperator{\Hom}{Hom} 
\DeclareMathOperator{\rank}{rank} 
\DeclareMathOperator{\Vol}{Vol}
\DeclareMathOperator{\Area}{Area}
\DeclareMathOperator{\dVol}{dVol}
\DeclareMathOperator{\supp}{supp} 
\DeclareMathOperator{\Int}{Int} 
\DeclareMathOperator{\Conv}{Conv} 
\DeclareMathOperator{\Cone}{Cone} 
\DeclareMathOperator{\Ker}{Ker} 
\DeclareMathOperator{\Span}{Span} 
\DeclareMathOperator{\Min}{Min} 
\newcommand{\bone}{\mathbf{1}}
\DeclareMathOperator{\tr}{tr} 
\newcommand{\bR}{\mathbb{R}} 
\newcommand{\bZ}{\mathbb{Z}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bK}{\mathbb{K}}
\newcommand{\bL}{\mathbb{L}} 
\newcommand{\bB}{\mathbb{B}} 
\newcommand{\bbT}{\mathbb{T}} 
\newcommand{\bN}{\mathbb{N}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cO}{\mathcal{O}} 
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cKG}{\mathcal{KG}}
\renewcommand{\phi}{\varphi}
\renewcommand{\div}{\mbox{div}}
\newcommand{\ve}{\varepsilon}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\ov}[1]{\overline{#1}}
\newcommand{\diff}[4]{\left.\left.\frac{\operatorname{d}}{\operatorname{d}#1}\right.^{#2}#3\right|_{#4}}
\renewcommand{\geq}{\geqslant}
\renewcommand{\leq}{\leqslant}
\renewcommand{\ge}{\geqslant}
\renewcommand{\le}{\leqslant}

\newcommand{\furlp}[1]{\colorbox{blue!10}{\href{run:/home/fulong/academia/library/papers/#1.pdf}{D}}}
\newcommand{\furlb}[1]{\colorbox{blue!10}{\href{run:/home/fulong/academia/library/books/#1.pdf}{D}}}
\newcommand{\fcitep}[1]{\cite{#1}\mbox{\furlp{#1}}}
\newcommand{\fciteb}[1]{\cite{#1}\mbox{\furlb{#1}}}
% we can now use cite as before
% misc defines
\newcommand{\energy}{U}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\hbx}{\hat{\mathbf{x}}}
\newcommand{\bbx}{\bar{\mathbf{x}}}
\newcommand{\sbx}{\mathbf{x}^{\star}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\hbb}{\hat{\mathbf{b}}}
\newcommand{\hbn}{\hat{\mathbf{n}}}
\newcommand{\bbb}{\bar{\mathbf{b}}}
\newcommand{\hbu}{\hat{\mathbf{u}}}
\newcommand{\bbu}{\bar{\mathbf{u}}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\mN}{\mathcal{N}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\mO}{\mathcal{O}}
\newcommand{\mP}{\mathcal{P}}
\newcommand{\mB}{\mathcal{B}}
\newcommand{\mC}{\mathcal{C}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mZ}{\mathcal{Z}}
\newcommand{\mW}{\mathcal{W}}
\newcommand{\mQ}{\mathcal{Q}}
\newcommand{\mR}{\mathcal{R}}
\newcommand{\mU}{\mathcal{U}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\mK}{\mathcal{K}}
\newcommand{\mV}{\mathcal{V}}
\newcommand{\mI}{\mathcal{I}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\hmX}{\hat{\mathcal{X}}}
\newcommand{\hmU}{\hat{\mathcal{U}}}
\newcommand{\bmX}{\bar{\mathcal{X}}}
\newcommand{\bmU}{\bar{\mathcal{U}}}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mM}{\mathcal{M}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\hbpsi}{\hat{\boldsymbol \psi}}
\newcommand{\bPsi}{\boldsymbol \Psi}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\sS}[1]{\sqrt{\Sigma_{#1}}}
\newcommand{\shS}[1]{\sqrt{\hat{\Sigma}_{#1}}}
\newcommand{\sd}{\texttt{sd}}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Tr}{tr}
\DeclareMathOperator{\st}{s.t.}
\DeclareMathOperator{\dt}{dt}
\DeclareMathOperator{\Vect}{vec}
\DeclareMathOperator{\diag}{diag}
%\DeclareMathOperator{\argmin}{arg\,min}

\newcommand{\specialcell}[2][c]{ \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\limit}[1] {\underset{#1}{\text{lim }}}
\newcommand{\infimum}[1] {\underset{#1}{\text{inf }}}
\newcommand{\supremum}[1] {\underset{#1}{\text{sup }}}
\newcommand{\maximum}[1] {\underset{#1}{\text{max }}}
\newcommand{\minimum}[1] {\underset{#1}{\text{min }}}
\newcommand{\myargmax}[1] {\underset{#1}{\text{argmax }}}
\newcommand{\myargmin}[1] {\underset{#1}{\text{argmin }}}
\newcommand{\expect}[1] {\mathbb{E}\left[#1\right]}

\newcommand{\TODO}[1]{\todo{#1}}


